A Theoretical Framework for Distribution-Aware Dataset Search

Effective data discovery is a cornerstone of modern data-driven decision-making. Yet, identifying datasets with specific distributional characteristics, such as percentiles or preferences, remains challenging. While recent proposals have enabled users to search based on percentile predicates, much of the research in data discovery relies on heuristics. This paper presents the first theoretically backed framework that unifies data discovery under centralized and decentralized settings. Let $\mathcal{P}=\{P_1,...,P_N\}$ be a repository of $N$ datasets, where $P_i\subset \mathbb{R}^d$, for $d=O(1)$ . We study the percentile indexing (Ptile) problem and the preference indexing (Pref) problem under the centralized and the federated setting. In the centralized setting we assume direct access to the datasets. In the federated setting we assume access to a synopsis of each dataset. The goal of Ptile is to construct a data structure such that given a predicate (rectangle $R$ and interval $\theta$) report all indexes $J$ such that $j\in J$ iff $|P_j\cap R|/|P_j|\in\theta$. The goal of Pref is to construct a data structure such that given a predicate (vector $v$ and interval $\theta$) report all indexes $J$ such that $j\in J$ iff $\omega(P_j,v)\in \theta$, where $\omega(P_j,v)$ is the inner-product of the $k$-th largest projection of $P_j$ on $v$. We first show that we cannot hope for near-linear data structures with polylogarithmic query time in the centralized setting. Next we show $\tilde{O}(N)$ space data structures that answer Ptile and Pref queries in $\tilde{O}(1+OUT)$ time, where $OUT$ is the output size. Each data structure returns a set of indexes $J$ such that i) for every $P_i$ that satisfies the predicate, $i\in J$ and ii) if $j\in J$ then $P_j$ satisfies the predicate up to an additive error $\varepsilon+2\delta$, where $\varepsilon\in(0,1)$ and $\delta$ is the error of synopses.

==> introduction.tex <==
\section{Problem Statement}

\rahul{I was thinking maybe we can choose not to define schema and attributes and directly define datasets to be point-sets in $\Re^d$. I suppose if we were interested in keyword queries, those would be more relevant. In the introduction ,we can say in words that we expect datasets in a repository to have common attributes...blah blah. I won't have time to make edits but if everyone agrees, someone please make the change }

\paragraph{Dataset}
A \emph{schema} $\A = (A_1, A_2, \ldots, A_d)$ is an ordered tuple of attributes.\footnote{We skip the formal definition of an attribute.} A \emph{dataset} $\DS$ with schema $\A$ is a finite set of data entries, where each entry $p\in \DS$ is a $d$-tuple $p = (p_1, p_2, \ldots, p_d)$ such that $p_i \in \dom(A_i)$ for $i = 1, 2, \ldots, d$. Thus, $\DS \subseteq \dom(A_1) \times \dom(A_2) \times \cdots \times \dom(A_d)$. In this paper, we focus on datasets where all attributes are numerical, i.e., $\dom(A_i) = \mathbb{R}$ for all $i$. Hence, $\DS \subset \mathbb{R}^d$. We denote the schema of a dataset $\DS$ as $\textsc{Schema}(\DS)$.


\paragraph{Repository} A \emph{repository} \(\Rep\) is a collection of datasets \(\Rep = \{\DS_1, \DS_2, \ldots, \DS_{\setsize}\}\), all of which share the same schema, i.e., \(\textsc{Schema}(\DS_i) = \textsc{Schema}(\DS_j)\) for all \(i, j\).
 \footnote{The assumption that all datasets contain only numerical attributes and share the same schema is not strictly required. These assumptions are adopted to simplify the presentation. For our framework to be applicable, it suffices for datasets in $\Rep$ to share at least some numerical attributes. }  



\paragraph{Measure Function}  A \emph{measure function} \(\M(\cdot)\), is a function that, when applied to a dataset \(\DS\), assigns a numerical value \(\M(\DS) \in \mathbb{R}\) to quantify a specific property or characteristic of the dataset. We assume that \(\M(\cdot)\) is applied to a dataset \(\DS\) only if \(\M(\DS)\) is well-defined. For example, a simple measure function is the \emph{dataset cardinality}, \(\M_{\text{card}}(\DS) = |\DS|\). 

\par A set of measure functions that quantify similar properties is called a \emph{class}, which we typically denote by \(\F\). In this paper, we will consider the following classes of measure functions:




\begin{enumerate} 
    \item \paragraph{Class of Percentile Measure Functions} Let \(\DS \subset \mathbb{R}^d\) be a dataset and let \(\rect\) be an axis-parallel rectangle in \(\mathbb{R}^d\). A \emph{percentile measure function} \(\M_{\rect}\) is defined as:
\[
\M_\rect(\DS) := \frac{| \rect \cap \DS |}{| \DS |},
\]. Interpreting \(\DS\) as a uniform discrete probability distribution with support defined by the points in $\DS$, \(\M_\rect(\DS)\) measures the mass of the distribution in the region \(\rect\). We denote the class of axis-parallel percentile measure functions in $\Re^d$ by:
\[
\F^d_{\Box} = \{\M_{\rect}(\cdot) \mid \rect \text{ is an axis-aligned rectangle in } \mathbb{R}^d\}.
\]

Thus, functions in $ \F^d_{\Box}$ can be used to measure the mass of a dataset $\DS$ in any rectangular-region.
\rahul{Application?}

 \medskip

    \item \paragraph{Class of Top-k Measure Functions} Let \(\DS \subset \mathbb{R}^d\) be a dataset. For a unit vector \(\vector \in \mathbb{R}^d\) and a point \(p \in \DS\), define the score of point $p$ with respect to vector $\vector$ as \(\score(p, \vector) = \langle p, \vector \rangle\), i.e., the inner product of \(p\) with \(\vector\). For an integer \(k > 0\), let \(\score_k(\DS, \vector)\) denote the score of the point in \(\DS\) with the \(k\)-th largest inner-product with respect to \(\vector\). A \emph{top-k measure function} is defined as:
\[
\M_{\vector,k}(\DS) := \score_k(\DS, \vector).
\]
In other words, \(\M_{\vector,k}(\DS)\) measures the \(k\)-th largest projection of points in \(\DS\) along the direction of \(\vector\). We denote the class of top-k measure functions in $\Re^d$ by 

\[
\vec{\F}^d_k = \{\M_{\vector,k}(\cdot) \mid \vector \text{ is a unit-vector in } \mathbb{R}^d\}.
\]

Thus, functions in $ \vec{\F}^d_{k}$ can be used to measure the $k$-th largest projection of the points in $\DS$ in any direction.
\rahul{Application?}
\end{enumerate}

 
\paragraph{Predicates} A \emph{predicate} \(\pred(\cdot)\) is a function that, given a dataset \(\DS\), evaluates to a truth value: \(\pred(\DS) \in \{\textsf{True}, \textsf{False}\}\). For a measure function \(\M\) and an interval \(\theta = [a, b]\), where \(a, b \in \mathbb{R}\) and \(a \leq b\), a \emph{range-predicate} \(\pred_{\M, \theta}(\DS)\) returns \textsf{True} if \(\M(\DS) \in \theta\). If $\theta$ is a one-sided interval (for instance, $\theta=[a,\infty)$), we call \(\pred_{\M, \theta}(\cdot)\) a \emph{threshold-predicate}. 
\par For example, for a dataset \(\DS \subset \mathbb{R}^d\) and a percentile measure \(\M_\rect\), \(\pred_{\M_{\rect}, \theta}(\DS)\) evaluates to \textsf{True} if the fraction of the dataset's mass within \(\rect\) lies in the range \(\theta\). Similarly, if \(\theta = [a, \infty)\), and the measure function is \(\M_{\vector, k}\), then \(\pred_{\M_{\vector, k}, \theta}(\DS)\) evaluates to \textsf{True} if there are at least \(k\) points in \(\DS\) whose inner product with \(\vector\) is at least \(a\), i.e., \(\score_k(\DS, \vector) \geq a\).

\par Complex predicates can be formed by combining individual predicates using conjunctions, disjunctions, and negations. For example, consider the complex predicate \(\Pi = \pred_{\M_{\rect_1, \theta_1}} \land \pred_{\M_{\rect_2, \theta_2}}\). The expression \(\Pi(\DS)\) evaluates to \textsf{True} if and only if both \(\pred_{\M_{\rect_1, \theta_1}}(\DS)\) and \(\pred_{\M_{\rect_2, \theta_2}}(\DS)\) are \textsf{True}, meaning the fraction of \(\DS\) within \(\rect_1\) lies in \(\theta_1\) and the fraction within \(\rect_2\) lies in \(\theta_2\).
In this work, we focus on complex predicates among measure functions of the same class, i.e., either all of them are percentile measure functions or top-$k$ measure functions.



% \paragraph{Range-Predicate} A \emph{predicate} $\pred(\cdot)$ is a function that, given a dataset $\DS$, evaluates to a truth value: $\pred(\DS) \in \{\textsf{True}, \textsf{False}\}$. For a measure function $\M$ and an interval $\theta=[a,b]$, where $a,b\in\Re$ and $a\leq b$, a range-predicate $\pred_{\M, \theta}(\DS)$  returns \textsf{True} if $\M(\DS) \in \theta$.
% \par For example, for a dataset \(\DS \subset \mathbb{R}^d\), and a percentile measure \( \M_\rect\), \(\pred_{\M_{\rect}, \theta}(\DS)\) evaluates to \textsf{True} if the fraction of the dataset's mass within \(\perc\) lies in the range \(\theta\).

% \par Similarly, if $\theta=[a,\infty]$, and the measure function is $\M_{\vector,k}$, then $\pred_{\M_{\vector,k},\theta}(\DS)$ evaluates to \textsf{true} if there are at least $k$ points in $\P$ whose inner-product with $\vector$ as value at least $a$, i.e. $\score_k(\DS,\vector)\geq a$.


\paragraph{Synopsis}
Let $\F$ be a class of measure functions. For a dataset $\DS$, a \emph{synopsis} (or \emph{sketch}) with respect to the class $\F$, denoted by $ \Synop_{\DS}^{\F}$, is a compressed representation of $\DS$ that captures the structure of $\DS$ with regards to the class $\F$. Ideally, for any function $\M \in \F$, \(
\M(\DS) \approx \M(\Synop_{\DS}^{\F}),
\)  where $\M(\Synop_{\DS}^{\F})$ is the result of evaluating the measure function $\M$ on $\Synop_{\DS}^{\F}$. \footnote{We assume $\M(\Synop_{\DS}^{\F})$ is well-defined.} 
We ignore the superscript and only write $\Synop_{\DS}$, when the class $\F$ is clear from context.
For a function $\M\in\F$, we denote the error of $\Synop_{\DS}$ on $\M$ as $\err_{\Synop_{\DS}}(\M)$, where the specific definition of  $\err_{\Synop_{\DS}}(\cdot)$ depends on the class $\F$ and the dataset $\DS$. We define $\err_{\Synop_{\DS}}(\F):=\max_{\M\in\F}\err_{\Synop_{\DS}}(\M)$. 

If \(\F = \F^d_{\Box}\), then commonly used synopses in practice include probability distributions over \(\mathbb{R}^d\), such as histograms \cite{}, mixture models \cite{}, and \(\varepsilon\)-samples
%(treated as discrete distributions)
~\cite{} (a formal definition of an $\eps$-sample is given in the next section).
The error in this context is defined as:
\[
\err_{\Synop_{\DS}}(\M_{\rect}) := |\M_{\rect}(\DS) - \M_{\rect}(\Synop_{\DS})|,
\]
where \(\M_{\rect}(\Synop_{\DS}) := \Pr_{p \sim \Synop_{\DS}}[p \in \rect]\), the probability that a point sampled according to the distribution defined by \(\Synop_{\DS}\) lies within the region \(\rect\). Consequently, \(\err_{\Synop_{\DS}}(\F^d_{\Box})\) is the maximum absolute difference between the values of \(\M_{\rect}(\DS)\) and \(\M_{\rect}(\Synop_{\DS})\) over all \(\M_{\rect} \in \F^d_{\Box}\).

\par If \(\F = \vec{\F}^d_{k}\), a $(k,\varepsilon)$-kernel~\cite{yu2012processing} of the dataset is commonly used as a synopsis in practice (a formal definition of $(k,\eps)$-kernel is given in the next section).
The error in this context is defined as:
\[
\err_{\Synop_{\DS}}(\M_{\vector,k}) := \M_{\vector,k}(\DS)-\M_{\vector,k}(\Synop_{\DS})
\]


\paragraph{Structure-Aware Indexing} Let \(\Rep = \{\DS_1, \DS_2, \ldots, \DS_{\setsize}\}\) be a repository, where each dataset \(\DS_i \subseteq \mathbb{R}^d\), and let \(\F\) be a class of measure functions. The general \emph{structure-aware indexing problem} for $(\Rep,\F)$ aims to design an index \(\I\) that, given a logical expression \(\Pi\) (of constant size) involving predicates of the form \(\pred_{\M, \theta}\), where \(\M \in \F\) and \(\theta\) is an interval in \(\mathbb{R}\), efficiently computes the subset of datasets in \(\Rep\) that satisfy \(\Pi\). Formally, the index \(\I\) should answer a \emph{structure-aware dataset query} \(\query_{\Pi}\):
\[
\query_\Pi(\Rep):= \{\DS_i \in \Rep \mid \Pi(\DS_i) = \textsc{True}\}.
\]




\par There are two variants of the problem. In the first variant, called \emph{centralized structure-aware indexing}, we have direct access to all the datasets in \(\Rep\) for building \(\I\). In the second variant, called \emph{federated structure-aware indexing}, we do not have direct access to \(\Rep\). Instead, we have access to a collection of synopses \(\Rep_{\Synop} = \{\Synop_{\DS_1}, \Synop_{\DS_2}, \ldots, \Synop_{\DS_{\setsize}}\}\), where \(\Synop_{\DS_i}\) is a synopsis of \(\DS_i\) with respect to \(\F\).

\par It is evident that, \(\query_{\Pi}(\Rep)\) can be answered exactly in the centralized setting, where direct access to all datasets in \(\Rep\) is available. Write more!!!

\par In the federated setting, however, the ability to evaluate  \(\Pi(\DS_i)\), for any $i$, critically depends on the quality of the synopsis \(\Synop_{\DS_i}\) provided for each dataset \(\DS_i\). Specifically, the ability to correctly decide any predicate \(\pred_{\M_j, \theta_j}(\DS_i)\) is influenced by the error \(\err_{\Synop_{\DS_i}}(\M_j)\), which is a measure of deviation between \(\M_j(\Synop_{\DS_i})\) and  \(\M_j(\DS_i)\). Hence, in the federated setting, 
our objective in determining \(\query_{\Pi}(\Rep)\) is to achieve an accuracy level that aligns with the fidelity of the provided synopses. If the synopsis \(\Synop_{\DS_i}\) accurately represents the dataset \(\DS_i\), our approach should ensure that the evaluation of \(\Pi(\DS_i)\) is similarly accurate for \(\DS_i\).

\par For the class of measure functions $\F^d_{\Box}$, this problem is better known in the literature as \emph{distribution-aware indexing} \cite{}, and the corresponding queries are referred to as a \emph{distribution-aware dataset queries} \cite{}. \rahul{Sainyam, can you add here?}

\par For the class of measure functions $\vec{\F}^d_{k}$, we call the problem \probTopk-aware indexing and the corresponding queries \probTopk-aware dataset queries \rahul{Sainyam, can you add here?}



\paragraph{Our Results}
We establish lower bounds and design efficient indexes for centralized and federated distribution-aware indexing and ?-aware indexing.


\begin{enumerate} [label=(\roman*)]
    \item \textit{Distribution-aware indexing}: Let $\Rep = \{\DS_1, \ldots, \DS_{\setsize}\}$ be a repository with $\setsize$ datasets, where each $\DS_i \subset \mathbb{R}^d$. Let $M = \sum_{\points_i \in \Rep} |\points_i|$ denote the total size of the datasets in $\Rep$. Let $\mathcal{F}^d_{\Box}$ be the class of percentile measures in $\mathbb{R}^d$. 

In Section~\ref{}, we prove a conditional lower bound, showing that no centralized distribution-aware index of size $\Tilde{O}(M)$ can answer distribution-aware dataset queries in $\Tilde{O}(1)$ time (Theorem~\ref{}). Moreover, this lower bound holds even when the query has only one predicate. This result is based on the conjectured hardness of the strong set intersection problem~\cite{}. Motivated by this hardness, we explore approximate solutions. 


\par Interestingly, in the approximate setting, we design an algorithm to build an index that functions identically in both centralized and federated settings, under the assumption that each synopsis $\Synop_{\DS_i}$ in the federated setting is a probability distribution over $\mathbb{R}^d$, and there exists a mechanism to sample according to the synopsis-distribution. Note that, in all practical cases, synopses used for distribution-aware dataset queries are indeed distributions, and sampling is usually possible (e.g., histograms). \rahul{Sainyam ?}

We first study a simpler variant where the search query has only one predicate. In both the centralized and federated settings, we design an index of size \textbf{?} in time \textbf{?}. In the centralized setting, we prove the following guarantee: \textbf{(state guarantee here)}. 

In the federated setting, we obtain similar guarantees if the synopses are nice. Specifically, if we know that $\err_{\Synop_{\DS_i}} \leq \delta_i$ for all $i$, we ensure that \textbf{(state guarantee here)}. 

\textit{Optional:} If we do not have information about the quality of the synopses, we achieve a slightly weaker guarantee. We ensure that for $\Pi(\DS_i) = \textsf{No}$, we may include it only if \textbf{(condition here)}. On the other hand, if $\Pi(\DS_i) = \textsf{Yes}$, we exclude it only if \textbf{(condition here)}.
When the search query  is based on a conjuncion of predicates, we..


\item \textit{???-aware indexing}: for top-k

\end{enumerate}




==> letter.tex <==
\thispagestyle{empty}
\begin{center}
    \huge{Cover Letter}
\end{center}

We would like to thank the reviewers for their thoughtful and constructive comments, as well as for the opportunity to revise the paper. We made all the suggested changes based on the reviewers' comments, significantly improving the presentation of the paper.
We use \new{blue color} to highlight major changes in the revised version. The most important changes, as highlighted by the rebuttal, are the following.


\vspace{2mm}
\noindent {\color{red} {Implement structural changes proposed in the common part of the rebuttal (technical overview, running example, pseudocode, simplified expressions with details in the appendix)} }

\smallskip 
\noindent {\bf Response:} 
We made all the proposed changes.
\begin{itemize}
\item We added a detailed overview of every data structure in Sections~\ref{sec:Perc} and~\ref{sec:topK}. In particular we show the overview of the data structure for the \problemDI problem with a threshold predicate in Subsection~\ref{subsec:approxpercopenright}, the overview of the data structure for the \problemDI problem with a range predicate in Subsection~\ref{subsec:approxPercRangePred}, and the overview of the data structure for the \problemDIk problem at the beginning of Section~\ref{sec:topK}.

    \item We added a toy example for the \problemDI problem in $1$ dimension in Section~\ref{sec:Perc}, please check Figure~\ref{fig:all}. After the construction of each data structure in Section~\ref{sec:Perc}, we show the data structure is constructed in our example. Similarly, after the description of every query procedure in Section~\ref{sec:Perc}, we show how the query procedure is executed in our example. The new Figure~\ref{fig:all} is also used in the overview to motivate our methods.

    \item We added pseudocode for the construction and query procedure of all our data structures in Section~\ref{sec:Perc} and~\ref{sec:topK}. Please check Algorithms~\ref{alg:construction},~\ref{alg:query},~\ref{alg:Gconstruction},~\ref{alg:Gquery},~\ref{alg:Topkconstruction},~\ref{alg:Topkquery}.

    \item We simplified the expressions in the analysis of the data structures in Section~\ref{sec:Perc} assuming that $\eps$ is an arbitrarily small constant and $\prob=\frac{1}{\setsize}$ (the theoretical guarantees hold with high probability). The full analysis is shown in Appendix~\ref{appndx:secPerc}.
\end{itemize}

\vspace{2mm}
\noindent {\color{red} {New motivating example in the introduction} }

\smallskip 
\noindent {\bf Response:} We replaced our motivating example in Section~\ref{sec:intro} with a new one, as described in the rebuttal.

\vspace{2mm}
\noindent {\color{red} {Make further structural changes in Introduction according to their response R3.1 (as they see fit)} }


\smallskip 
\noindent {\bf Response:} We made all the structural changes to improve the presentation in Section~\ref{sec:intro}. More specifically:

\begin{itemize}
    \item We added Subsection~\ref{subsec:framework} describing a general framework that captures all practical problems in distribution-aware dataset search. This framework consists of a repository over datasets, a measure function, a predicate function, a synopsis and an error function. We also defined the centralized and federated settings of the framework. 

    \item Next, we added Subsection~\ref{subsec:probldef} defining two classes of measure functions that we study in this paper, namely the class of percentile measure functions, and the class of top-k preference measure functions. Then, we clearly define the Percentile-aware indexing problem (in both centralized and federated setting) and the Preference-aware indexing problem (in both centralized and federated setting), based on the pre-defined framework. 

    \item We made Subsection~\ref{sec:results} "Our Results" shorter highlighting only the main results. We also removed the repetitive summary of contributions from the introduction.
\end{itemize}



\vspace{2mm}
\noindent {\color{red} {Add an expanded discussion of future work.} }

\smallskip 
\noindent {\bf Response:} We extended the discussion of future work in Section~\ref{sec:concl} as proposed in the rebuttal. First, we discuss more distribution-aware dataset search problems that arise from how our framework. Then, we explain the main obstacle preventing our data structures from handling all such problems, and how our methods could help address it in the future.
%On the other hand, our work is the the first step toward efficiently solving such problems with theoretical guarantees.
%On the other hand, our new methods 
Furthermore, we discuss why the general \problemCDI problem in $1$-dimension is challenging and why our exact data structure for a fixed predicate (presented in Appendix~\ref{subsec:percExact}) cannot handle it. On the other hand, we explain how our method can be used to approach such a problem in the future.

\thispagestyle{empty}
\vspace{5mm}
\noindent Sincerely,\\
The authors


\newpage
\pagenumbering{arabic}
